An OpenMind for 3D medical vision self-supervised learning

The field of self-supervised learning (SSL) for 3D medical images lacks consistency and standardization. While many methods have been developed, it is impossible to identify the current state-of-the-art, due to i) varying and small pretraining datasets, ii) varying architectures, and iii) being evaluated on differing downstream datasets. In this paper, we bring clarity to this field and lay the foundation for further method advancements through three key contributions: We a) publish the largest publicly available pre-training dataset comprising 114k 3D brain MRI volumes, enabling all practitioners to pre-train on a large-scale dataset. We b) benchmark existing 3D self-supervised learning methods on this dataset for a state-of-the-art CNN and Transformer architecture, clarifying the state of 3D SSL pre-training. Among many findings, we show that pre-trained methods can exceed a strong from-scratch nnU-Net ResEnc-L baseline. Lastly, we c) publish the code of our pre-training and fine-tuning frameworks and provide the pre-trained models created during the benchmarking process to facilitate rapid adoption and reproduction.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

\usepackage{pgf}
\usepackage[table,xcdraw,dvipsnames]{xcolor}

\definecolor{goodred}{HTML}{e7638d}     % pink-red
\definecolor{goodyellow}{HTML}{f2e17c}  % soft yellow (midpoint)
\definecolor{goodgreen}{HTML}{a1d76a}   % lime-green


\newcommand{\definecolorrange}[5]{%
    \expandafter\newcommand\csname colorrange#1#2#3\endcsname[1]{%
        \pgfmathsetmacro{\minval}{#4}  % Set dataset-specific min value
        \pgfmathsetmacro{\maxval}{#5}  % Set dataset-specific max value
        \pgfmathsetmacro{\midval}{(\minval+\maxval)/2}  % Compute midpoint

        \pgfmathsetmacro{\PercentColor}{100.0*(##1-\minval)/(\maxval-\minval)}%
        \ifdim ##1 pt < \minval pt
            \cellcolor{goodred}{##1}%
        \else
            \ifdim ##1 pt > \maxval pt
                \cellcolor{goodgreen}{##1}%
            \else
                \ifdim ##1 pt < \midval pt
                    \pgfmathsetmacro{\PercentLow}{200.0*(##1-\minval)/(\maxval-\minval)}%
                    \xdef\PercentLow{\PercentLow}%
                    \cellcolor{goodyellow!\PercentLow!goodred}{##1}%
                \else
                    \pgfmathsetmacro{\PercentHigh}{200.0*(##1-\midval)/(\maxval-\minval)}%
                    \xdef\PercentHigh{\PercentHigh}%
                    \cellcolor{goodgreen!\PercentHigh!goodyellow}{##1}%
                \fi
            \fi
        \fi
    }
}

\definecolorrange{ATL}{cnn}{bench}{56.07}{58.76}
\definecolorrange{SBM}{cnn}{bench}{53.43}{64.09}
\definecolorrange{ISL}{cnn}{bench}{77.45}{79.14}
\definecolorrange{HNT}{cnn}{bench}{59.37}{66.58}
\definecolorrange{HAN}{cnn}{bench}{45}{55.14}
\definecolorrange{MSF}{cnn}{bench}{52.19}{57.42}
\definecolorrange{TPC}{cnn}{bench}{74.69}{79.94}
\definecolorrange{YBM}{cnn}{bench}{54.42}{60.07}
\definecolorrange{COS}{cnn}{bench}{46.10}{71.57}
\definecolorrange{ACD}{cnn}{bench}{90.72}{92.09}
\definecolorrange{AMO}{cnn}{bench}{83.88}{88.0}
\definecolorrange{KIT}{cnn}{bench}{77.61}{87.48}
\definecolorrange{IDMean}{cnn}{bench}{58.33}{65.11}
\definecolorrange{OODMean}{cnn}{bench}{84.07}{88.30}
\definecolorrange{Mean}{cnn}{bench}{64.77}{70.91}

% Additional definitions for transformer models
\definecolorrange{ATL}{trans}{bench}{46.80}{61.16}
\definecolorrange{SBM}{trans}{bench}{34.15}{56.67}
\definecolorrange{ISL}{trans}{bench}{73.29}{77.54}
\definecolorrange{HNT}{trans}{bench}{50.15}{66.12}
\definecolorrange{HAN}{trans}{bench}{46.49}{57.24}
\definecolorrange{MSF}{trans}{bench}{53.27}{56.02}
\definecolorrange{TPC}{trans}{bench}{65.52}{78.31}
\definecolorrange{YBM}{trans}{bench}{43}{54.35}
\definecolorrange{COS}{trans}{bench}{51.16}{72.02}
\definecolorrange{ACD}{trans}{bench}{87.27}{92.16}
\definecolorrange{AMO}{trans}{bench}{65.81}{87.24}
\definecolorrange{KIT}{trans}{bench}{70.21}{86.74}
\definecolorrange{IDMean}{trans}{bench}{52.00}{64.34}
\definecolorrange{OODMean}{trans}{bench}{74.43}{88.69}
\definecolorrange{Mean}{trans}{bench}{57.61}{70.42}

% Additional definitions for transformer models
\definecolorrange{ATL}{cnn}{onek}{56.64}{61.04}
\definecolorrange{SBM}{cnn}{onek}{53.43}{62.35}
\definecolorrange{ISL}{cnn}{onek}{77.24}{79.14}
\definecolorrange{HNT}{cnn}{onek}{60.83}{65.75}
\definecolorrange{HAN}{cnn}{onek}{53.37}{59.48}
\definecolorrange{MSF}{cnn}{onek}{52.19}{55.08}
\definecolorrange{TPC}{cnn}{onek}{76.17}{79.94}
\definecolorrange{YBM}{cnn}{onek}{56.12}{60.24}
\definecolorrange{COS}{cnn}{onek}{46.19}{72.24}
\definecolorrange{ACD}{cnn}{onek}{91.10}{92.11}
\definecolorrange{AMO}{cnn}{onek}{88.00}{88.86}
\definecolorrange{KIT}{cnn}{onek}{87.21}{88.24}
\definecolorrange{IDMean}{cnn}{onek}{61.08}{65.6134}
\definecolorrange{OODMean}{cnn}{onek}{88.77}{89.67}
\definecolorrange{Mean}{cnn}{onek}{68.00}{71.63}

% Substract this offset from the second worst DSC
\newcommand\offset{1}

% CNN FINETUNING SCHEDULES

\definecolorrange{SBM}{VoCo}{cnn}{70.26-\offset}{73.86}
\definecolorrange{ATL}{VoCo}{cnn}{59.32-\offset}{62.78}
\definecolorrange{AMO}{VoCo}{cnn}{85.91-\offset}{86.98}
\definecolorrange{KIT}{VoCo}{cnn}{84.08-\offset}{85.80}
\definecolorrange{AVG}{VoCo}{cnn}{74.92-\offset}{77.09}
\definecolorrange{SBM}{SwinUNETR}{cnn}{69.16-\offset}{71.05}
\definecolorrange{ATL}{SwinUNETR}{cnn}{60.23-\offset}{61.17}
\definecolorrange{AMO}{SwinUNETR}{cnn}{85.42-\offset}{86.61}
\definecolorrange{KIT}{SwinUNETR}{cnn}{81.77-\offset}{83.83}
\definecolorrange{AVG}{SwinUNETR}{cnn}{74.44-\offset}{75.31}
\definecolorrange{SBM}{SimCLR}{cnn}{72.79-\offset}{73.94}
\definecolorrange{ATL}{SimCLR}{cnn}{57.95-\offset}{62.36}
\definecolorrange{AMO}{SimCLR}{cnn}{86.72-\offset}{87.12}
\definecolorrange{KIT}{SimCLR}{cnn}{81.20-\offset}{83.10}
\definecolorrange{AVG}{SimCLR}{cnn}{74.48-\offset}{76.30}
\definecolorrange{SBM}{VF}{cnn}{72.57-\offset}{75.81}
\definecolorrange{ATL}{VF}{cnn}{63.20-\offset}{65.07}
\definecolorrange{AMO}{VF}{cnn}{86.05-\offset}{86.58}
\definecolorrange{KIT}{VF}{cnn}{83.51-\offset}{85.41}
\definecolorrange{AVG}{VF}{cnn}{76.60-\offset}{77.84}
\definecolorrange{SBM}{MG}{cnn}{73.37-\offset}{74.68}
\definecolorrange{ATL}{MG}{cnn}{61.23-\offset}{63.46}
\definecolorrange{AMO}{MG}{cnn}{86.93-\offset}{87.34}
\definecolorrange{KIT}{MG}{cnn}{83.48-\offset}{84.15}
\definecolorrange{AVG}{MG}{cnn}{76.62-\offset}{77.36}
\definecolorrange{SBM}{MAE}{cnn}{71.84-\offset}{74.79}
\definecolorrange{ATL}{MAE}{cnn}{62.78-\offset}{63.61}
\definecolorrange{AMO}{MAE}{cnn}{86.78-\offset}{87.62}
\definecolorrange{KIT}{MAE}{cnn}{83.48-\offset}{85.24}
\definecolorrange{AVG}{MAE}{cnn}{76.49-\offset}{77.75}
\definecolorrange{SBM}{SD}{cnn}{72.40-\offset}{75.47}
\definecolorrange{ATL}{SD}{cnn}{62.16-\offset}{63.76}
\definecolorrange{AMO}{SD}{cnn}{86.45-\offset}{87.54}
\definecolorrange{KIT}{SD}{cnn}{82.20-\offset}{83.78}
\definecolorrange{AVG}{SD}{cnn}{76.40-\offset}{76.87}
\definecolorrange{SBM}{Mean}{cnn}{72.82-\offset}{73.23}
\definecolorrange{ATL}{Mean}{cnn}{61.68-\offset}{62.40}
\definecolorrange{AMO}{Mean}{cnn}{86.42-\offset}{86.69}
\definecolorrange{KIT}{Mean}{cnn}{83.32-\offset}{84.09}
\definecolorrange{AVG}{Mean}{cnn}{76.15-\offset}{76.60}

% TRANSFORMER FINETUNING SCHEDULES

\definecolorrange{SBM}{VoCo}{TR}{37.55-\offset}{44.16}
\definecolorrange{ATL}{VoCo}{TR}{48.04-\offset}{48.53}
\definecolorrange{AMO}{VoCo}{TR}{66.01-\offset}{67.71}
\definecolorrange{KIT}{VoCo}{TR}{66.33-\offset}{68.31}
\definecolorrange{AVG}{VoCo}{TR}{54.64-\offset}{57.98}
\definecolorrange{SBM}{SwinUNETR}{TR}{41.64-\offset}{47.65}
\definecolorrange{ATL}{SwinUNETR}{TR}{47.72-\offset}{48.87}
\definecolorrange{AMO}{SwinUNETR}{TR}{66.51-\offset}{67.96}
\definecolorrange{KIT}{SwinUNETR}{TR}{68.00-\offset}{69.13}
\definecolorrange{AVG}{SwinUNETR}{TR}{56.42-\offset}{58.10}
\definecolorrange{SBM}{SimCLR}{TR}{54.11-\offset}{59.92}
\definecolorrange{ATL}{SimCLR}{TR}{51.97-\offset}{56.60}
\definecolorrange{AMO}{SimCLR}{TR}{75.88-\offset}{76.42}
\definecolorrange{KIT}{SimCLR}{TR}{77.47-\offset}{80.58}
\definecolorrange{AVG}{SimCLR}{TR}{65.38-\offset}{68.38}
\definecolorrange{SBM}{VF}{TR}{64.12-\offset}{66.03}
\definecolorrange{ATL}{VF}{TR}{63.00-\offset}{63.66}
\definecolorrange{AMO}{VF}{TR}{84.81-\offset}{85.73}
\definecolorrange{KIT}{VF}{TR}{80.40-\offset}{83.02}
\definecolorrange{AVG}{VF}{TR}{73.14-\offset}{74.31}
\definecolorrange{SBM}{MG}{TR}{59.11-\offset}{62.95}
\definecolorrange{ATL}{MG}{TR}{57.81-\offset}{59.43}
\definecolorrange{AMO}{MG}{TR}{82.91-\offset}{83.12}
\definecolorrange{KIT}{MG}{TR}{80.00-\offset}{82.00}
\definecolorrange{AVG}{MG}{TR}{70.14-\offset}{71.51}
\definecolorrange{SBM}{MAE}{TR}{66.88-\offset}{70.86}
\definecolorrange{ATL}{MAE}{TR}{60.95-\offset}{61.48}
\definecolorrange{AMO}{MAE}{TR}{87.80-\offset}{87.93}
\definecolorrange{KIT}{MAE}{TR}{86.29-\offset}{86.45}
\definecolorrange{AVG}{MAE}{TR}{75.39-\offset}{76.78}
\definecolorrange{SBM}{SimMIM}{TR}{66.16-\offset}{68.10}
\definecolorrange{ATL}{SimMIM}{TR}{59.80-\offset}{60.74}
\definecolorrange{AMO}{SimMIM}{TR}{87.79-\offset}{88.22}
\definecolorrange{KIT}{SimMIM}{TR}{83.78-\offset}{85.54}
\definecolorrange{AVG}{SimMIM}{TR}{74.50-\offset}{75.58}
\definecolorrange{SBM}{Mean}{TR}{56.30-\offset}{59.67}
\definecolorrange{ATL}{Mean}{TR}{56.07-\offset}{56.76}
\definecolorrange{AMO}{Mean}{TR}{78.90-\offset}{79.51}
\definecolorrange{KIT}{Mean}{TR}{77.86-\offset}{79.08}
\definecolorrange{AVG}{Mean}{TR}{67.42-\offset}{68.76}

% Below are the color ranges using the min. and max. values of each block. However, the frozen encoder DSC values are way too low compared to 
% the other learning rate schedules, resulting in a table filled with only green colors (except for the red rows corresponding to the frozen encoder).

% % CNN FINETUNING SCHEDULES

% \definecolorrange{SBM}{VoCo}{cnn}{52.34}{73.86}
% \definecolorrange{ATL}{VoCo}{cnn}{58.27}{62.78}
% \definecolorrange{AMO}{VoCo}{cnn}{53.18}{86.98}
% \definecolorrange{KIT}{VoCo}{cnn}{69.33}{85.80}
% \definecolorrange{AVG}{VoCo}{cnn}{58.28}{77.09}
% \definecolorrange{SBM}{SwinUNETR}{cnn}{38.59}{71.05}
% \definecolorrange{ATL}{SwinUNETR}{cnn}{54.27}{61.17}
% \definecolorrange{AMO}{SwinUNETR}{cnn}{61.26}{86.61}
% \definecolorrange{KIT}{SwinUNETR}{cnn}{69.59}{83.83}
% \definecolorrange{AVG}{SwinUNETR}{cnn}{55.93}{75.31}
% \definecolorrange{SBM}{SimCLR}{cnn}{60.83}{73.94}
% \definecolorrange{ATL}{SimCLR}{cnn}{56.80}{62.36}
% \definecolorrange{AMO}{SimCLR}{cnn}{62.92}{87.12}
% \definecolorrange{KIT}{SimCLR}{cnn}{65.22}{83.10}
% \definecolorrange{AVG}{SimCLR}{cnn}{61.73}{76.30}
% \definecolorrange{SBM}{VF}{cnn}{28.54}{75.81}
% \definecolorrange{ATL}{VF}{cnn}{43.33}{65.07}
% \definecolorrange{AMO}{VF}{cnn}{30.97}{86.58}
% \definecolorrange{KIT}{VF}{cnn}{36.06}{85.41}
% \definecolorrange{AVG}{VF}{cnn}{34.73}{77.84}
% \definecolorrange{SBM}{MG}{cnn}{51.35}{74.68}
% \definecolorrange{ATL}{MG}{cnn}{57.27}{63.46}
% \definecolorrange{AMO}{MG}{cnn}{57.89}{87.34}
% \definecolorrange{KIT}{MG}{cnn}{71.39}{84.15}
% \definecolorrange{AVG}{MG}{cnn}{59.48}{77.36}
% \definecolorrange{SBM}{MAE}{cnn}{59.45}{74.79}
% \definecolorrange{ATL}{MAE}{cnn}{54.49}{63.61}
% \definecolorrange{AMO}{MAE}{cnn}{50.83}{87.62}
% \definecolorrange{KIT}{MAE}{cnn}{63.97}{85.24}
% \definecolorrange{AVG}{MAE}{cnn}{57.18}{77.75}
% \definecolorrange{SBM}{SD}{cnn}{56.55}{75.47}
% \definecolorrange{ATL}{SD}{cnn}{57.15}{63.76}
% \definecolorrange{AMO}{SD}{cnn}{52.48}{87.54}
% \definecolorrange{KIT}{SD}{cnn}{71.41}{83.78}
% \definecolorrange{AVG}{SD}{cnn}{59.40}{76.87}
% \definecolorrange{SBM}{Mean}{cnn}{49.67}{73.23}
% \definecolorrange{ATL}{Mean}{cnn}{54.68}{62.40}
% \definecolorrange{AMO}{Mean}{cnn}{52.79}{86.69}
% \definecolorrange{KIT}{Mean}{cnn}{63.85}{84.09}
% \definecolorrange{AVG}{Mean}{cnn}{55.25}{76.60}

% % TRANSFORMER FINETUNING SCHEDULES

% \definecolorrange{SBM}{VoCo}{TR}{18.56}{44.16}
% \definecolorrange{ATL}{VoCo}{TR}{25.88}{48.53}
% \definecolorrange{AMO}{VoCo}{TR}{10.23}{67.28}
% \definecolorrange{KIT}{VoCo}{TR}{22.02}{68.31}
% \definecolorrange{AVG}{VoCo}{TR}{19.17}{57.98}
% \definecolorrange{SBM}{SwinUNETR}{TR}{21.50}{47.65}
% \definecolorrange{ATL}{SwinUNETR}{TR}{28.99}{48.87}
% \definecolorrange{AMO}{SwinUNETR}{TR}{12.73}{67.96}
% \definecolorrange{KIT}{SwinUNETR}{TR}{24.14}{69.13}
% \definecolorrange{AVG}{SwinUNETR}{TR}{21.84}{58.10}
% \definecolorrange{SBM}{SimCLR}{TR}{25.26}{59.92}
% \definecolorrange{ATL}{SimCLR}{TR}{39.90}{56.60}
% \definecolorrange{AMO}{SimCLR}{TR}{21.52}{76.42}
% \definecolorrange{KIT}{SimCLR}{TR}{33.67}{80.58}
% \definecolorrange{AVG}{SimCLR}{TR}{30.09}{68.38}
% \definecolorrange{SBM}{VF}{TR}{39.78}{66.03}
% \definecolorrange{ATL}{VF}{TR}{32.91}{63.66}
% \definecolorrange{AMO}{VF}{TR}{10.74}{85.73}
% \definecolorrange{KIT}{VF}{TR}{23.87}{83.02}
% \definecolorrange{AVG}{VF}{TR}{26.83}{74.31}
% \definecolorrange{SBM}{MG}{TR}{34.62}{62.95}
% \definecolorrange{ATL}{MG}{TR}{47.18}{59.43}
% \definecolorrange{AMO}{MG}{TR}{29.40}{83.12}
% \definecolorrange{KIT}{MG}{TR}{33.10}{82.00}
% \definecolorrange{AVG}{MG}{TR}{36.07}{71.51}
% \definecolorrange{SBM}{MAE}{TR}{46.83}{70.86}
% \definecolorrange{ATL}{MAE}{TR}{57.57}{61.48}
% \definecolorrange{AMO}{MAE}{TR}{37.67}{87.93}
% \definecolorrange{KIT}{MAE}{TR}{40.82}{86.45}
% \definecolorrange{AVG}{MAE}{TR}{45.72}{76.78}
% \definecolorrange{SBM}{SimMIM}{TR}{43.74}{68.10}
% \definecolorrange{ATL}{SimMIM}{TR}{49.59}{60.74}
% \definecolorrange{AMO}{SimMIM}{TR}{11.02}{88.22}
% \definecolorrange{KIT}{SimMIM}{TR}{27.40}{85.54}
% \definecolorrange{AVG}{SimMIM}{TR}{32.94}{75.58}
% \definecolorrange{SBM}{Mean}{TR}{32.90}{59.67}
% \definecolorrange{ATL}{Mean}{TR}{40.29}{56.76}
% \definecolorrange{AMO}{Mean}{TR}{19.04}{79.51}
% \definecolorrange{KIT}{Mean}{TR}{29.29}{79.08}
% \definecolorrange{AVG}{Mean}{TR}{30.38}{68.76}


% ADDED CNN DATACENTRIC RESULT
\definecolorrange{ATL}{cnn}{data}{58.25}{59.33}
\definecolorrange{SBM}{cnn}{data}{62.41}{65.21}
\definecolorrange{ISL}{cnn}{data}{77.89}{78.57}
\definecolorrange{HNT}{cnn}{data}{65.80}{66.58}
\definecolorrange{HAN}{cnn}{data}{51.06}{55.14}
\definecolorrange{MSF}{cnn}{data}{56.24}{57.42}
\definecolorrange{TPC}{cnn}{data}{77.17}{79.00}
\definecolorrange{YBM}{cnn}{data}{59.12}{60.28}
\definecolorrange{COS}{cnn}{data}{68.90}{73.37}
\definecolorrange{ACD}{cnn}{data}{91.98}{92.11}
\definecolorrange{AMO}{cnn}{data}{86.57}{86.78}
\definecolorrange{KIT}{cnn}{data}{85.66}{86.20}
\definecolorrange{IDMean}{cnn}{data}{64.58}{65.31}
\definecolorrange{OODMean}{cnn}{data}{88.13}{88.30}
\definecolorrange{Mean}{cnn}{data}{70.48}{71.05}


% CLASSIFICATION TABLE RESULT
\definecolorrange{MRNet}{cnn}{AP}{66.33}{71.99}
\definecolorrange{RSNASpine}{cnn}{AP}{65.39}{71.21}
\definecolorrange{ABIDE}{cnn}{AP}{57.18}{62.32}
\definecolorrange{Mean}{cnn}{AP}{62.97}{68.18}
\definecolorrange{MRNet}{cnn}{BalAcc}{76.61}{80.35}
\definecolorrange{RSNASpine}{cnn}{BalAcc}{62.25}{67.96}
\definecolorrange{ABIDE}{cnn}{BalAcc}{53.29}{60.18}
\definecolorrange{Mean}{cnn}{BalAcc}{65.80}{66.58}
\definecolorrange{MRNet}{tr}{AP}{60.58}{68.86}
\definecolorrange{RSNASpine}{tr}{AP}{58.91}{62.09}
\definecolorrange{ABIDE}{tr}{AP}{52.41}{56.84}
\definecolorrange{Mean}{tr}{AP}{57.45}{62.14}
\definecolorrange{MRNet}{tr}{BalAcc}{75.49}{77.73}
\definecolorrange{RSNASpine}{tr}{BalAcc}{57.10}{61.64}
\definecolorrange{ABIDE}{tr}{BalAcc}{51.28}{56.06}
\definecolorrange{Mean}{tr}{BalAcc}{61.55}{63.94}


\newcommand{\alldatasetcite}[0]{\nocite{ds000001:1.0.0,ds000109:2.0.2,ds000170:00001,ds000220:1.0.0,ds000245:00001,ds001226:5.0.0,ds001365:1.0.0,ds001511:1.0.5,ds001614:1.1.0,ds001780:1.0.0,ds001928:1.1.0,ds002144:2.0.0,ds002295:1.0.0,ds002425:1.0.2,ds002672:1.0.0,ds002738:1.0.2,ds002842:1.0.1,ds003017:1.0.3,ds003126:1.3.1,ds003357:1.0.0,ds003441:1.0.0,ds003500:1.2.0,ds003606:1.0.0,ds003715:1.0.0,ds003799:2.0.0,ds003950:1.0.0,ds004073:1.0.1,ds004146:1.0.4,ds004271:1.1.0,ds004400:1.0.6,ds004489:1.0.1,ds004589:1.0.0,ds004663:1.0.4,ds004746:1.0.1,ds004869:1.1.1,ds004993:1.1.2,ds005088:1.0.0,ds005237:1.1.3,ds005374:1.0.1,ds005525:1.0.0,ds000002:00002,ds000171:00001,ds000246:1.0.1,ds001371:1.1.1,ds001621:1.1.0,ds001942:1.2.0,ds002306:1.1.0,ds002674:1.0.6,ds002843:1.0.1,ds003136:1.0.0,ds003442:1.0.0,ds003612:1.0.4,ds003814:1.0.0,ds004078:1.2.1,ds004274:1.0.0,ds004493:1.0.2,ds004666:1.0.5,ds004873:2.0.6,ds005096:1.0.3,ds005375:1.0.0,ds000003:1.0.0,ds000005:00001,ds000006:00001,ds000007:00001,ds000008:00001,ds000009:00002,ds000011:1.0.0,ds000017:00001,ds000030:1.0.0,ds000031:2.0.2,ds000051:00001,ds000052:00001,ds000053:00001,ds000101:00004,ds000102:00001,ds000105:3.0.0,ds000107:00001,ds000108:00002,ds000110:00001,ds000113:1.3.0,ds000114:1.0.2,ds000115:00001,ds000116:00003,ds000117:1.1.0,ds000119:00001,ds000120:00001,ds000121:00001,ds000122:00001,ds000133:00001,ds000140:00001,ds000144:00002,ds000148:1.0.0,ds000149:1.0.0,ds000157:00001,ds000158:1.0.0,ds000164:00001,ds000168:1.0.0,ds000172:1.0.1,ds000174:1.0.1,ds000200:00001,ds000201:1.0.3,ds000202:00001,ds000203:00001,ds000204:00002,ds000205:00001,ds000206:1.0.0,ds000208:1.0.1,ds000210:00002,ds000212:1.0.0,ds000213:00002,ds000214:00001,ds000216:00001,ds000217:1.0.0,ds000218:00002,ds000219:00001,ds000221:1.0.0,ds000222:1.0.1,ds000223:00001,ds000224:1.0.4,ds000228:1.1.1,ds000229:00001,ds000231:1.0.0,ds000232:00001,ds000233:1.0.1,ds000234:00002,ds000235:2.0.1,ds000236:2.0.1,ds000237:1.0.0,ds000238:00002,ds000239:00001,ds000240:2.0.0,ds000241:00002,ds000243:00001,ds000244:1.0.0,ds000247:1.0.2,ds000248:1.2.4,ds000249:00002,ds000253:00002,ds000254:1.0.0,ds000255:00002,ds000256:00002,ds000258:1.0.1,ds001021:1.0.0,ds001037:00001,ds001105:00001,ds001110:00003,ds001131:1.0.0,ds001132:1.0.0,ds001145:1.0.0,ds001168:1.0.1,ds001178:00002,ds001218:00001,ds001228:00002,ds001229:1.0.1,ds001232:1.0.0,ds001233:00003,ds001235:00001,ds001241:1.0.1,ds001242:1.0.0,ds001246:1.2.1,ds001247:00001,ds001297:00001,ds001299:1.0.0,ds001302:1.0.1,ds001306:1.0.0,ds001338:1.0.0,ds001339:00003,ds001344:1.0.0,ds001345:1.0.0,ds001353:1.0.0,ds001357:00001,ds001379:1.0.0,ds001386:00001,ds001399:2.0.0,ds001408:1.0.3,ds001415:1.0.0,ds001417:1.0.0,ds001419:1.0.1,ds001420:1.2.0,ds001421:1.4.1,ds001430:1.0.2,ds001439:1.2.0,ds001454:1.3.1,ds001486:1.3.1,ds001491:1.0.0,ds001497:1.0.2,ds001499:1.3.1,ds001506:1.3.1,ds001510:2.0.3,ds001517:1.0.3,ds001521:1.0.2,ds001525:1.1.1,ds001534:1.1.0,ds001545:1.1.1,ds001551:1.0.0,ds001553:1.0.1,ds001554:1.0.0,ds001555:1.0.1,ds001563:1.0.1,ds001566:1.0.1,ds001576:1.0.0,ds001590:1.0.1,ds001595:1.0.0,ds001597:1.0.0,ds001600:1.0.0,ds001607:1.0.1,ds001608:1.0.1,ds001612:1.0.2,ds001634:1.0.1,ds001635:1.0.1,ds001652:2.0.0,ds001705:1.0.1,ds001715:1.0.0,ds001722:1.1.0,ds001728:1.1.0,ds001734:1.0.5,ds001740:2.2.0,ds001743:1.0.1,ds001745:1.1.0,ds001747:1.1.0,ds001748:1.0.4,ds001751:1.0.2,ds001761:2.0.1,ds001762:1.0.1,ds001771:1.0.2,ds001775:1.0.1,ds001784:1.1.2,ds001796:1.7.0,ds001814:1.0.7,ds001818:1.0.0,ds001832:1.0.1,ds001838:1.0.1,ds001839:1.0.1,ds001840:1.0.2,ds001847:1.0.1,ds001848:1.0.1,ds001882:1.0.7,ds001883:1.0.3,ds001894:1.4.2,ds001907:3.1.0,ds001912:1.0.2,ds001921:1.0.0,ds001923:1.0.0,ds001926:1.0.1,ds001927:2.1.0,ds001946:1.0.3,ds001972:1.0.2,ds001978:1.0.3,ds001984:1.0.2,ds002000:1.0.0,ds002001:1.0.0,ds002006:1.0.1,ds002011:1.0.0,ds002013:1.0.3,ds002014:1.0.1,ds002016:1.0.0,ds002033:1.0.1,ds002040:1.0.2,ds002041:2.0.0,ds002076:1.0.1,ds002080:4.0.0,ds002105:1.1.0,ds002116:1.0.0,ds002149:1.0.5,ds002153:1.0.1,ds002155:1.0.0,ds002156:2.0.0,ds002158:1.0.2,ds002168:1.1.0,ds002169:1.0.0,ds002185:1.1.0,ds002207:1.0.0,ds002232:1.0.0,ds002236:1.1.1,ds002237:1.1.0,ds002241:1.1.1,ds002242:1.0.0,ds002250:1.0.1,ds002270:1.0.0,ds002278:2.0.0,ds002293:1.0.0,ds002294:1.0.1,ds002311:1.1.0,ds002316:1.0.0,ds002320:1.1.0,ds002322:1.0.4,ds002328:1.0.2,ds002330:1.1.0,ds002336:2.0.2,ds002338:2.0.2,ds002345:1.1.4,ds002363:1.1.1,ds002366:1.1.0,ds002367:1.0.0,ds002380:1.0.1,ds002382:1.0.1,ds002411:1.1.0,ds002419:1.0.3,ds002422:1.1.0,ds002424:1.2.0,ds002513:1.0.0,ds002522:1.0.2,ds002543:1.0.1,ds002547:1.1.0,ds002549:1.0.1,ds002550:1.0.1,ds002574:1.0.1,ds002578:1.1.0,ds002596:1.0.1,ds002603:1.0.0,ds002606:1.1.0,ds002608:1.0.2,ds002609:1.0.3,ds002614:1.0.0,ds002620:1.0.0,ds002634:3.0.0,ds002643:1.1.0,ds002647:1.0.1,ds002655:1.0.1,ds002675:1.0.0,ds002684:1.0.0,ds002685:2.0.0,ds002687:1.2.0,ds002702:1.0.1,ds002711:1.1.0,ds002712:1.0.1,ds002715:1.0.0,ds002717:1.0.1,ds002725:1.0.0,ds002726:1.0.1,ds002727:1.0.2,ds002731:1.0.2,ds002732:1.0.0,ds002733:1.0.1,ds002734:1.0.2,ds002735:1.0.2,ds002737:1.0.1,ds002739:1.0.0,ds002741:1.0.2,ds002743:1.0.1,ds002748:1.0.5,ds002750:1.0.1,ds002766:3.0.2,ds002770:2.0.0,ds002773:1.0.0,ds002776:1.0.2,ds002785:2.0.0,ds002790:2.0.0,ds002793:1.0.1,ds002797:1.0.2,ds002799:1.0.4,ds002813:1.0.0,ds002814:1.3.0,ds002835:1.0.1,ds002837:2.0.0,ds002841:1.0.1,ds002848:1.0.1,ds002872:1.3.0,ds002878:2.0.0,ds002879:1.1.1,ds002886:1.1.0,ds002896:1.0.0,ds002898:1.4.2,ds002905:1.0.1,ds002936:1.0.0,ds002938:1.0.1,ds002940:1.0.1,ds002979:1.0.0,ds002989:1.0.0,ds002994:1.0.3,ds002995:1.0.1,ds003007:1.0.1,ds003011:1.2.3,ds003012:1.0.4,ds003020:3.0.0,ds003037:2.1.0,ds003043:1.0.0,ds003047:1.0.0,ds003059:1.0.0,ds003076:1.0.1,ds003078:1.0.0,ds003082:1.0.1,ds003083:1.0.1,ds003085:1.0.0,ds003089:1.0.1,ds003094:1.0.0,ds003095:1.0.0,ds003096:1.0.2,ds003097:1.2.1,ds003098:1.0.0,ds003103:1.0.1,ds003104:1.0.0,ds003114:1.0.1,ds003138:1.0.1,ds003145:1.0.2,ds003146:1.0.2,ds003148:1.0.1,ds003151:2.0.1,ds003170:2.0.0,ds003171:2.0.1,ds003176:2.0.1,ds003192:1.0.1,ds003216:3.0.11,ds003233:1.2.1,ds003242:1.0.0,ds003338:1.1.0,ds003340:1.0.4,ds003342:1.0.0,ds003345:1.0.2,ds003346:1.1.2,ds003354:1.0.1,ds003358:1.0.0,ds003367:1.0.0,ds003381:1.0.1,ds003382:1.5.0,ds003392:1.0.4,ds003397:1.2.3,ds003401:1.0.1,ds003404:1.0.5,ds003416:2.0.2,ds003424:1.0.0,ds003425:1.0.2,ds003430:1.2.0,ds003433:1.0.1,ds003434:1.0.1,ds003436:1.0.0,ds003437:1.0.2,ds003438:1.0.0,ds003439:1.0.0,ds003440:1.0.0,ds003443:1.0.0,ds003444:1.0.0,ds003445:1.0.0,ds003446:1.0.0,ds003452:1.0.1,ds003453:1.0.4,ds003454:1.0.1,ds003455:1.0.2,ds003459:1.0.2,ds003465:1.0.7,ds003466:1.1.1,ds003469:1.0.0,ds003470:2.0.0,ds003481:1.0.3,ds003484:1.0.0,ds003487:2.0.0,ds003495:1.0.0,ds003499:1.0.1,ds003505:1.1.2,ds003507:1.0.1,ds003508:1.0.0,ds003511:1.1.2,ds003521:2.2.0,ds003524:1.0.0,ds003540:1.0.1,ds003542:1.0.0,ds003545:1.0.0,ds003548:1.0.1,ds003550:1.0.2,ds003553:1.0.2,ds003554:1.0.3,ds003563:1.1.0,ds003568:1.0.4,ds003569:1.0.0,ds003574:1.0.2,ds003592:1.0.13,ds003604:1.0.7,ds003633:1.0.4,ds003639:1.0.0,ds003642:1.1.0,ds003643:2.0.7,ds003653:1.0.0,ds003659:2.0.4,ds003661:1.0.0,ds003669:1.0.0,ds003673:2.0.1,ds003684:1.0.0,ds003688:1.0.7,ds003691:1.0.0,ds003696:1.0.0,ds003701:1.0.1,ds003707:1.0.0,ds003709:1.0.0,ds003711:1.0.0,ds003714:1.0.1,ds003716:1.0.0,ds003717:1.1.0,ds003720:1.0.1,ds003721:1.0.1,ds003745:2.1.1,ds003752:1.0.0,ds003758:1.0.2,ds003763:1.0.5,ds003764:1.0.5,ds003768:1.0.11,ds003770:1.2.1,ds003772:1.0.1,ds003777:1.0.1,ds003778:1.0.0,ds003782:1.0.1,ds003787:1.0.1,ds003789:2.0.0,ds003791:1.0.0,ds003798:1.0.5,ds003823:1.3.5,ds003826:3.0.1,ds003831:1.0.0,ds003834:1.0.2,ds003835:1.0.2,ds003836:1.0.0,ds003848:1.0.3,ds003849:1.0.0,ds003851:1.0.1,ds003858:1.0.1,ds003871:1.0.2,ds003872:1.0.0,ds003877:1.1.1,ds003892:5.0.0,ds003900:1.1.1,ds003922:1.0.1,ds003927:1.0.1,ds003949:1.0.1,ds003965:1.0.0,ds003967:1.0.0,ds003972:1.0.0,ds003974:3.0.0,ds003988:1.0.0,ds003990:1.0.2,ds003993:1.0.0,ds003999:1.0.2,ds004006:1.0.4,ds004007:1.0.2,ds004009:1.0.0,ds004021:1.0.0,ds004024:1.0.1,ds004038:1.0.0,ds004042:1.0.1,ds004044:2.0.3,ds004054:1.0.0,ds004056:1.0.2,ds004065:1.0.0,ds004081:1.0.0,ds004086:1.2.0,ds004091:2.0.0,ds004094:1.0.1,ds004097:1.1.0,ds004101:1.0.1,ds004102:1.0.1,ds004103:1.0.0,ds004107:1.0.0,ds004109:1.0.0,ds004128:1.0.0,ds004129:1.0.0,ds004130:1.0.0,ds004131:1.0.1,ds004134:1.0.1,ds004141:1.0.5,ds004142:1.0.1,ds004144:1.0.2,ds004158:2.0.5,ds004169:1.0.7,ds004173:1.0.2,ds004182:1.0.1,ds004187:1.0.2,ds004192:1.0.7,ds004194:2.0.0,ds004196:2.0.2,ds004199:1.0.6,ds004212:2.0.1,ds004213:1.0.1,ds005752:2.1.0,ds004217:1.0.0,ds004219:1.0.0,ds004226:1.0.0,ds004228:1.0.1,ds004230:3.0.0,ds004259:1.0.0,ds004261:2.0.0,ds004280:1.0.1,ds004283:1.0.3,ds004285:1.0.0,ds004286:1.0.0,ds004299:1.0.0,ds004301:1.0.2,ds004302:1.0.1,ds004312:1.0.3,ds004323:1.0.0,ds004327:1.0.3,ds004331:1.0.4,ds004332:1.3.0,ds004341:1.0.0,ds004346:1.0.8,ds004349:1.0.0,ds004359:1.0.0,ds004392:1.0.0,ds004393:1.0.4,ds004401:1.3.0,ds004406:1.0.0,ds004440:1.0.1,ds004443:1.0.0,ds004450:1.0.1,ds004455:1.1.0,ds004456:1.0.1,ds004458:1.0.2,ds004466:1.0.2,ds004467:1.0.0,ds004469:1.1.4,ds004470:1.0.1,ds004471:1.0.1,ds004473:1.0.2,ds004475:1.0.3,ds004478:1.0.2,ds004482:1.0.0,ds004484:1.0.1,ds004488:1.1.1,ds004496:2.1.2,ds004498:1.0.0,ds004499:1.0.3,ds004505:1.0.4,ds004513:1.0.4,ds004516:2.0.2,ds004529:1.1.1,ds004533:1.0.0,ds004539:1.1.1,ds004542:1.0.0,ds004544:1.0.0,ds004553:1.0.1,ds004556:1.0.1,ds004557:1.1.0,ds004560:1.0.1,ds004562:1.0.4,ds004564:1.0.1,ds004581:2.0.1,ds004590:1.0.0,ds004592:1.0.1,ds004594:1.0.1,ds004597:2.0.0,ds004604:2.0.0,ds004605:1.0.1,ds004611:1.0.2,ds004627:1.1.0,ds004630:1.1.3,ds004631:1.0.0,ds004636:1.0.4,ds004640:1.0.4,ds004645:1.0.0,ds004647:1.0.2,ds004648:1.0.0,ds004650:1.0.2,ds004654:1.0.1,ds004656:1.1.0,ds004662:1.1.0,ds004670:1.0.1,ds004692:1.0.0,ds004693:1.0.3,ds004697:1.0.2,ds004698:2.0.1,ds004710:1.1.0,ds004711:1.0.0,ds004712:2.0.1,ds004715:1.0.3,ds004717:1.0.0,ds004718:1.1.1,ds004720:1.0.0,ds004725:1.0.1,ds004730:1.0.0,ds004731:1.0.0,ds004733:1.0.0,ds004737:2.0.0,ds004743:1.0.0,ds004765:1.0.0,ds004775:1.1.1,ds004776:1.0.0,ds004783:1.0.1,ds004786:1.0.1,ds004787:1.1.0,ds004791:1.0.0,ds004795:1.0.0,ds004798:1.0.5,ds004808:1.0.0,ds004814:1.0.0,ds004815:1.0.1,ds004829:1.0.1,ds004835:1.0.0,ds004837:1.0.0,ds004848:1.0.1,ds004856:1.2.0,ds004866:1.0.0,ds004868:1.0.4,ds004884:1.0.2,ds004889:1.1.2,ds004892:1.0.1,ds004894:1.0.0,ds004909:1.1.0,ds004910:1.0.1,ds004917:1.0.1,ds004920:1.1.1,ds004928:1.0.0,ds004934:1.0.0,ds005754:1.1.0,ds004937:1.0.1,ds004945:1.0.0,ds004946:1.0.0,ds004956:1.0.1,ds004957:1.0.2,ds004958:1.0.0,ds004965:1.0.1,ds004996:2.0.0,ds005003:2.0.0,ds005009:1.0.0,ds005012:1.0.3,ds005016:1.1.1,ds005017:1.0.2,ds005026:1.0.0,ds005027:1.0.3,ds005038:1.0.3,ds005040:1.2.0,ds005047:1.0.7,ds005050:1.0.0,ds005056:1.0.0,ds005063:1.0.0,ds005069:1.0.0,ds005072:1.0.1,ds005073:1.0.0,ds005075:1.0.1,ds005085:1.0.0,ds005115:1.2.0,ds005118:1.0.0,ds005123:1.1.3,ds005125:1.0.0,ds005126:1.0.3,ds005127:1.0.4,ds005128:1.0.0,ds005134:1.0.0,ds005139:1.0.7,ds005148:1.1.0,ds005165:1.0.4,ds005169:1.0.0,ds005191:1.0.2,ds005194:1.1.0,ds005215:1.0.0,ds005216:1.1.0,ds005230:1.0.0,ds005234:2.1.7,ds005239:1.0.1,ds005250:1.1.5,ds005261:2.0.2,ds005263:1.0.0,ds005264:1.0.0,ds005265:1.0.0,ds005266:1.0.0,ds005267:1.0.1,ds005279:1.0.3,ds005295:1.0.2,ds005299:1.0.0,ds005304:1.0.3,ds005355:1.0.1,ds005357:1.0.0,ds005360:1.0.0,ds005364:1.0.0,ds005365:1.0.1,ds005366:2.0.0,ds005371:1.1.3,ds005381:1.0.0,ds005386:1.0.0,ds005401:1.1.1,ds005412:1.0.0,ds005415:1.0.0,ds005418:3.2.0,ds005422:1.0.1,ds005427:1.1.1,ds005449:1.0.0,ds005454:1.0.0,ds005455:1.1.5,ds005464:1.0.1,ds005469:2.0.0,ds005479:1.0.3,ds005492:1.0.0,ds005498:2.0.0,ds005504:1.0.0,ds005518:1.0.1,ds005529:1.0.1,ds005530:1.0.9,ds005531:1.0.0,ds005533:1.0.0,ds005559:1.0.1,ds005571:1.0.1,ds005573:1.0.0,ds005576:1.0.0,ds005581:1.0.0,ds005588:1.0.0,ds005595:1.0.0,ds005596:1.1.1,ds005597:1.0.1,ds005598:1.0.0,ds005600:1.1.0,ds005602:1.0.0,ds005603:1.0.1,ds005604:1.0.1,ds005619:1.1.0}}

==> tables/modality_counts.tex <==
\begin{tabular}{llr}
\toprule
 & modality & count \\
\midrule
0 & T1w & 42732 \\
1 & T2w & 22999 \\
2 & FA & 13407 \\
3 & MD & 13407 \\
4 & FLAIR & 5583 \\
5 & MP2RAGE & 2859 \\
6 & sbref & 1795 \\
7 & ADC & 1757 \\
8 & TRACE & 1715 \\
9 & UNIT1 & 927 \\
10 & inplaneT2 & 892 \\
11 & SWI & 784 \\
12 & UNIT1_denoised & 724 \\
13 & minIP & 687 \\
14 & PET & 653 \\
15 & T1map & 557 \\
16 & inplaneT1 & 529 \\
17 & angio & 488 \\
18 & PDw & 473 \\
19 & T2starw & 409 \\
20 & FLASH & 307 \\
21 & T2map & 106 \\
22 & T2starmap & 76 \\
23 & DWI & 55 \\
\bottomrule
\end{tabular}


==> tables/test_results_tr.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
Dataset & nnU-Net fix. & VoCo & SwinUNETR & VF & MG & MAE & SimMIM \\
\midrule
ATLAS & 51.51\% & 45.88\% & 47.07\% & 58.64\% & 56.60\% & 60.67\% & 60.85\% \\
SBM & 43.26\% & 32.13\% & 33.21\% & 47.74\% & 45.93\% & 54.98\% & 51.63\% \\
ISLES22 & 75.23\% & 73.86\% & 73.77\% & 77.40\% & 76.34\% & 77.93\% & 76.47\% \\
HNTS-MRG & 55.30\% & 49.79\% & 49.75\% & 61.35\% & 59.25\% & 65.96\% & 65.99\% \\
HaN-Seg MR & 50.60\% & 47.11\% & 45.54\% & 53.91\% & 54.12\% & 57.76\% & 56.61\% \\
MS-FLAIR & 54.00\% & 51.42\% & 51.45\% & 54.97\% & 54.60\% & 55.75\% & 54.97\% \\
ToP-CoW & 73.31\% & 64.73\% & 65.27\% & 73.77\% & 72.25\% & 77.87\% & 77.92\% \\
YBM & 50.30\% & 43.84\% & 43.01\% & 53.95\% & 49.75\% & 54.43\% & 53.77\% \\
COSMOS & 62.11\% & 46.15\% & 54.36\% & 65.21\% & 63.83\% & 73.41\% & 69.80\% \\\midrule
ACDC & 90.93\% & 86.65\% & 87.33\% & 91.50\% & 91.15\% & 92.18\% & 92.16\% \\
AMOS22 & 80.17\% & 63.23\% & 63.89\% & 84.16\% & 81.54\% & 86.77\% & 87.08\% \\
KiTS23 & 76.73\% & 66.23\% & 68.62\% & 86.05\% & 84.08\% & 87.07\% & 86.53\% \\\midrule
ID Mean & 57.29\% & 50.55\% & 51.49\% & 60.77\% & 59.19\% & 64.31\% & 63.11\% \\
OOD MEAN & 82.61\% & 72.04\% & 73.28\% & 87.23\% & 85.59\% & 88.67\% & 88.59\% \\
Mean & 63.62\% & 55.92\% & 56.94\% & 67.39\% & 65.79\% & 70.40\% & 69.48\% \\
\bottomrule
\end{tabular}


==> tables/test_results_tr_transposed.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrr}
\toprule
Dataset & ATL & SBM & ISL & HNT & HAN & MSF & TPC & YBM & COS & ACD & AMO & KIT & IID & OOD & All \\
PT Method &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
nnU-Net fix. & 51.51 & 43.26 & 75.23 & 55.30 & 50.60 & 54.00 & 73.31 & 50.30 & 62.11 & 90.93 & 80.17 & 76.73 & 57.29 & 82.61 & 63.62 \\
VoCo & 45.88 & 32.13 & 73.86 & 49.79 & 47.11 & 51.42 & 64.73 & 43.84 & 46.15 & 86.65 & 63.23 & 66.23 & 50.55 & 72.04 & 55.92 \\
SwinUNETR & 47.07 & 33.21 & 73.77 & 49.75 & 45.54 & 51.45 & 65.27 & 43.01 & 54.36 & 87.33 & 63.89 & 68.62 & 51.49 & 73.28 & 56.94 \\
VF & 58.64 & 47.74 & 77.40 & 61.35 & 53.91 & 54.97 & 73.77 & 53.95 & 65.21 & 91.50 & 84.16 & 86.05 & 60.77 & 87.23 & 67.39 \\
MG & 56.60 & 45.93 & 76.34 & 59.25 & 54.12 & 54.60 & 72.25 & 49.75 & 63.83 & 91.15 & 81.54 & 84.08 & 59.19 & 85.59 & 65.79 \\
MAE & 60.67 & 54.98 & 77.93 & 65.96 & 57.76 & 55.75 & 77.87 & 54.43 & 73.41 & 92.18 & 86.77 & 87.07 & 64.31 & 88.67 & 70.40 \\
SimMIM & 60.85 & 51.63 & 76.47 & 65.99 & 56.61 & 54.97 & 77.92 & 53.77 & 69.80 & 92.16 & 87.08 & 86.53 & 63.11 & 88.59 & 69.48 \\
\bottomrule
\end{tabular}

